A standardisation proof for algebraic pattern calculi

This work gives some insights and results on standardisation for call-by-name pattern calculi. More precisely, we define standard reductions for a pattern calculus with constructor-based data terms and patterns. This notion is based on reduction steps that are needed to match an argument with respect to a given pattern. We prove the Standardisation Theorem by using the technique developed by Takahashi and Crary for lambda-calculus. The proof is based on the fact that any development can be specified as a sequence of head steps followed by internal reductions, i.e. reductions in which no head steps are involved.

==> eptcsdata.tex <==
\providecommand{\firstpage}{58}
\providecommand{\publicationstatus}{E. Bonelli (Ed.): 5th International Workshop\\
on Higher-Order Rewriting (HOR'10)\\
EPTCS 49, 2011, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.49.5}{10.4204/EPTCS.49.5}}

